Detecting sub-populations in online health communities: A mixed-methods exploration of breastfeeding messages in BabyCenter Birth Clubs

Parental stress is a nationwide health crisis according to the U.S. Surgeon General's 2024 advisory. To allay stress, expecting parents seek advice and share experiences in a variety of venues, from in-person birth education classes and parenting groups to virtual communities, for example, BabyCenter, a moderated online forum community with over 4 million members in the United States alone. In this study, we aim to understand how parents talk about pregnancy, birth, and parenting by analyzing 5.43M posts and comments from the April 2017--January 2024 cohort of 331,843 BabyCenter "birth club" users (that is, users who participate in due date forums or "birth clubs" based on their babies' due dates). Using BERTopic to locate breastfeeding threads and LDA to summarize themes, we compare documents in breastfeeding threads to all other birth-club content. Analyzing time series of word rank, we find that posts and comments containing anxiety-related terms increased steadily from April 2017 to January 2024. We used an ensemble of topic models to identify dominant breastfeeding topics within birth clubs, and then explored trends among all user content versus those who posted in threads related to breastfeeding topics. We conducted Latent Dirichlet Allocation (LDA) topic modeling to identify the most common topics in the full population, as well as within the subset breastfeeding population. We find that the topic of sleep dominates in content generated by the breastfeeding population, as well anxiety-related and work/daycare topics that are not predominant in the full BabyCenter birth club dataset.

==> bin/countcheckboxes-total <==
#!/usr/bin/perl

undef $/;
    $counts=0;
foreach $file (@ARGV) {
    open (FILE, "$file") or die "can't open $file: $!\n";

    $text = <FILE>;
    while ($text =~ m/\\todo{/g) {
	$counts++;
    }
    close FILE;
}
print "$counts";


==> bin/rename <==
#!/usr/bin/perl

$usage = "rename text1 text2 file [files...]

swap text1 for text2 in file names
whenever text1 is found.

swaps only the first instance.

rudimentary first version: use only for static text.
";

$pattern1 = $ARGV[0];
$pattern2 = $ARGV[1];

foreach $filename (@ARGV[2..$#ARGV]) {
    if ($filename =~ m/$pattern1/) {
	($newfilename = $filename) =~ s/$pattern1/$pattern2/g;
	print "renaming $filename as $newfilename...\n";
	`mv "$filename" "$newfilename"`;
    }
}


==> correspondence/2017-01-13pre.body.tex <==
%% rob axtell
%% sid redner
%% neil johnson
%% martin gerlach
%% newman?
%% simon dideo
%% aaron clauset
%% dashun wang
%% y.-y. ahn
%% sune lehmann
%% luis amaral

To the Editors,

We are very pleased to submit our manuscript for consideration at
Physical Review E:\\
\textbf{``Simon's fundamental rich-gets-richer model entails a dominant first-mover advantage.''}

Simon's famous 1955 rich-gets-richer model is a fundamental
and elementary system-growth mechanism that leads to power-law 
size distributions of component sizes.  
Also known as cumulative advantage and preferential attachment in networks,
Simon's growth mechanism is of profound theoretical importance and widespread
application across complex systems of all kinds.

\textbf{Remarkably, we show that Simon's model has
been drastically misunderstood for over 60 years.}

In our manuscript, 
\textbf{we demonstrate that the first entrant into the system enjoys a first-mover advantage
completely missed in Simon's analysis and, from what we believe, all subsequent
work.}  Through simulations and theory, we show that 
the first-mover advantage is powerful with the size gap
growing as the inverse of the empirically small innovation rate.

As Figure 1 in our manuscript shows, the first mover may be
enormous and seemingly impossible to miss---yet this is what we
have discovered.

We also explore the dynamics of all groups showing the potential
for a high degree of unpredictability in a group's long term success,
connecting with similar observations in the literature.

\textbf{We provide empirical evidence from citation count data} that a pure Simon model
can be invoked to capture a real system with a clear first-mover advantage.

Our work calls into question all past empirical analysis of real-world
systems
using Simon's model
as well as much theoretical work,
and, in going forward, we provide possible adjustments to Simon's model to
better fit real-world data.

We note that we have received valuable feedback from a number of outstanding colleagues
after our initial posting on the arXiv and have improved the manuscript
substantially.

Our correspondents include:
\begin{itemize}
\item 
  Sidney Redner,
\item 
  James P.\ Gleeson,
\item 
  Mason A.\ Porter,
\item 
  Cesar A.\ Hidalgo,
\item 
  Matus Medo, and 
\item 
  Mark E.\ J.\ Newman.
\end{itemize}

\textbf{We believe our paper will be well received by a large and broad audience 
in the physics community and we hope will prove to 
be an important contribution in the years to come.} 


%% \textbf{1.}
%% \textbf{2.}
%% \textbf{3.}
%% \textbf{4.}

%% \textbf{}

We look forward to hearing of your decision.

Yours sincerely and on behalf of the manuscript's authors,


%% Professor
%% Director of the Vermont Complex Systems Center
%% Co-Director, Computational Story Lab
%% Vermont Advanced Computing Center
%% Department of Mathematics and Statistics
%% The University of Vermont


==> paper-template-revtex4.settings.tex <==
\newcommand{\filenamebase}{paper-template}


==> paper-template.biblio.tex <==
\bibliography{\filenamebase}


==> paper-template.changelog.tex <==
%% for arXivs of the various stripes

\todo{Notes on what has changed}


==> paper-template.keywords.tex <==
Keywords,
Line,
By Line


==> paper-template.methods.tex <==
\section{Methods}
\label{sec:papertag.methods}






==> paper-template.nutshell.tex <==
\todo{Write a 1--3 sentence nutshell (logline)}



==> paper-template.pacs.tex <==
\pacs{89.65.-s,89.75.Da,89.75.Fb,89.75.-k}

%% 89.65.-s	Social and economic systems
%% 89.75.Da	Systems obeying scaling laws
%% 89.75.Fb	Structures and organization in complex systems
%% 89.75.-k	Complex systems (for complex chemical systems, see 82.40.Qt; for biological complexity, see 87.18.-h)


